Deep Learning and Inverse Problems

Machine Learning (ML) methods and tools have gained great success in many data, signal, image and video processing tasks, such as classification, clustering, object detection, semantic segmentation, language processing, Human-Machine interface, etc. In computer vision, image and video processing, these methods are mainly based on Neural Networks (NN) and in particular Convolutional NN (CNN), and more generally Deep NN. Inverse problems arise anywhere we have indirect measurement. As, in general, those inverse problems are ill-posed, to obtain satisfactory solutions for them needs prior information. Different regularization methods have been proposed, where the problem becomes the optimization of a criterion with a likelihood term and a regularization term. The main difficulty, however, in great dimensional real applications, remains the computational cost. Using NN, and in particular Deep Learning (DL) surrogate models and approximate computation, can become very helpful. In this work, we focus on NN and DL particularly adapted for inverse problems. We consider two cases: First the case where the forward operator is known and used as physics constraint, the second more general data driven DL methods.

==> biblio/revuedef.tex <==
% TEX 7(ascii) bits
% fichier : revuedef.tex	Auteur: AMD, GLB	09/92
% Modifie et completee par	L.Lemitre le 05 10 94
%				et al...
%
% Ce fichier contient des alias sur les noms de revues
% pour faciliter la saisie de fiches biblio.
%
% En commentaire, le facteur d'impact (nombre moyen de citation
% des articles, normalise a la moyenne mondiale sur l'ensemble
% des revues indexees par ISI) pour l'annee 1994 (J. I.). 

\def\AsAs{Astrononmy and Astrophysics}					% 2.328
\def\AAP{Advances in Applied Probability}				% 0.549
\def\ABE{Annals of Biomedical Engineering}				% 0.709
\def\AISM{Annals of Institute of Statistical Mathematics}		% 0.175
\def\AMS{Annals of Mathematical Statistics}			% ANNALS OF MATHEMATICS STUDIES ? 0.8            
\def\AO{Applied Optics}							% 1.033
\def\AP{The Annals of Probability}					% 0.68
\def\ARAA{Annual Review of Astronomy and Astrophysics}			% 9.865
\def\AST{The Annals of Statistics}					% 0.78
\def\AT{Annales des T\'el\'ecommunications}				% 0.155
\def\BMC{Biometrics}							% 1.207
\def\BMK{Biometrika}							% 0.832
\def\CPAM{Communications on Pure and Applied Mathematics}		% 1.282
\def\EMK{Econometrica}							% 2.54
\def\CRAS{Compte-rendus de l'acad\'emie des sciences}			% ?
\def\CVGIP{Computer Vision and Graphics and Image Processing}		% ?
\def\GJRAS{Geophysical Journal of the Royal Astrononomical Society}	% 1.371
\def\GSC{Geoscience}						% GEOSCIENCE CANADA ? 0.273
\def\GPH{Geophysics}							% 0.824
\def\GRETSI#1{Actes du #1$^{\mbox{e}}$ Colloque GRETSI} 		% ?
\def\CGIP{Computer Graphics and Image Processing}			% ?
\def\ICASSP{Proceedings of IEEE ICASSP}					% ?
\def\ICEMBS{Proceedings of IEEE EMBS}					% ?
\def\ICIP{Proceedings of the International Conference on Image Processing}% ?
\def\ieeP{Proceedings of the IEE}					% ?
\def\ieeeAC{IEEE Transactions on Automatic and Control}			% 0.867
\def\ieeeAES{IEEE Transactions on Aerospace and Electronic Systems}	% 0.459
\def\ieeeAP{IEEE Transactions on Antennas and Propagation}		% 0.806
\def\ieeeAPm{IEEE Antennas and Propagation Magazine}			% ?
\def\ieeeASSP{IEEE Transactions on Acoustics Speech and Signal Processing}% ?
\def\ieeeBME{IEEE Transactions on Biomedical Engineering}		% 1.061
\def\ieeeCS{IEEE Transactions on Circuits and Systems}			% 0.54
\def\ieeeCT{IEEE Transactions on Circuit Theory}			% 0.732
\def\ieeeC{IEEE Transactions on Communications}				% 0.969
\def\ieeeGE{IEEE Transactions on Geoscience and Remote Sensing}		% 1.356
\def\ieeeGEE{IEEE Transactions on Geosciences Electronics}		% ?
\def\ieeeIP{IEEE Transactions on Image Processing}			% ?
\def\ieeeIT{IEEE Transactions on Information Theory}			% 1.971
\def\ieeeMI{IEEE Transactions on Medical Imaging}			% 1.372
\def\ieeeMTT{IEEE Transactions on Microwave Theory and Technology}	% 1.004
\def\ieeeM{IEEE Transactions on Magnetics}				% 0.758
\def\ieeeNS{IEEE Transactions on Nuclear Sciences}			% 1.183
\def\ieeePAMI{IEEE Transactions on Pattern Analysis and Machine Intelligence}% 2.006
\def\ieeeP{Proceedings of the IEEE}					% ?
\def\ieeeRS{IEEE Transactions on Radio Science}				% ?
\def\ieeeSMC{IEEE Transactions on Systems, Man and Cybernetics}		% 0.649
\def\ieeeSP{IEEE Transactions on Signal Processing}			% 1.234
\def\ieeeSSC{IEEE Transactions on Systems Science and Cybernetics}	% ?
\def\ieeeSU{IEEE Transactions on Sonics and Ultrasonics}		% ?
\def\ieeeUFFC{IEEE Transactions on Ultrasonics Ferroelectrics and Frequency Control}% 0.927
\def\IJC{International Journal of Control}				% 0.617
\def\IJCV{International Journal of Computer Vision}			% 1.153
\def\IJIST{International Journal of Imaging Systems and Technology}	% ?
\def\IP{Inverse Problems}						% 0.98
\def\ISR{International Statistical Review}				% 0.75
\def\IUSS{Proceedings of International Ultrasonics Symposium}		% ?
\def\JAPH{Journal of Applied Physics}					% 1.658
\def\JAP{Journal of Applied Probability}				% 0.432
\def\JAS{Journal of Applied Statistics}					% ?
\def\JASA{Journal of Acoustical Society America}			% 1.273
\def\JASAS{Journal of American Statistical Association}			% 1.244
\def\JBME{Journal of Biomedical Engineering}				% 0.7
\def\JCAM{Journal of Computational and Applied Mathematics}		% 0.349
\def\JEWA{Journal of Electromagnetic Waves and Applications}		% 0.514
\def\JMO{Journal of Modern Optics}					% 1.005
\def\JNDE{Journal of Nondestructive Evaluation}				% ?
\def\JMP{Journal of Mathematical Physics}				% 0.969
\def\JOSA{Journal of the Optical Society of America}			% 1.425 (A-OPTICS IMAGE SCIENCE AND VISION)
\def\JP{Journal de Physique}						% 1.773 JOURNAL DE PHYSIQUE I
									% 1.923 JOURNAL DE PHYSIQUE II
									% 0.475 JOURNAL DE PHYSIQUE III
									% 0.115 JOURNAL DE PHYSIQUE IV
\def\JRSSA{Journal of the Royal Statistical Society A}			% 0.976
\def\JRSSB{Journal of the Royal Statistical Society B}			% 2.538
\def\JRSSC{Journal of the Royal Statistical Society C}			% ?
\def\JSPI{Journal of Statistical Planning and Inference}  		% 0.145
\def\JTSA{Journal of Time Series Analysis}                   		% ?
\def\JVCIR{Journal of Visual Communication and Image Representation} 	% ?
	\def\MMAS{???} % Trouve dans gpi base 				% ?
\def\KAP{Kluwer \uppercase{A}cademic \uppercase{P}ublishers}							% 
\def\MNAS{Mathematical Methods in Applied Science}			% 0.247
\def\MNRAS{Monthly Notices of the Royal Astronomical Society}		% 3.089
\def\MP{Mathematical Programming}					% 0.763
	\def\NSIP{NSIP}  % Trouve dans gpi base				% ?
\def\OC{Optics Communication}						% 1.205
\def\PRA{Physical Review A}						% 2.292
\def\PRB{Physical Review B}						% 3.187
\def\PRC{Physical Review C}						% 1.842
\def\PRD{Physical Review D}						% 3.233
\def\PRL{Physical Review Letters}					% 6.626
\def\RGSP{Review of Geophysics and Space Physics}			% 4.314
\def\RPA{Revue de Physique Appliqu\'e}							% 0.753
\def\RS{Radio Science}							% 0.753
\def\SP{Signal Processing}						% 0.44
\def\siamAM{SIAM Journal of Applied Mathematics}			% 0.743
\def\siamCO{SIAM Journal of Control}					% 0.968
\def\siamJO{SIAM Journal of Optimization}				% ?
\def\siamMA{SIAM Journal of Mathematical Analysis}			% 0.765
\def\siamNA{SIAM Journal of Numerical Analysis}				% 1.021
\def\siamR{SIAM Review}							% 1.216
\def\SSR{Stochastics and Stochastics Reports}       			% ?
\def\TPA{Theory of Probability and its Applications}			% 0.045
\def\TMK{Technometrics}							% 1.585
\def\TS{Traitement du Signal}						% ?
\def\UCMMP{U.S.S.R. Computational Mathematics and Mathematical Physics}	% ?
\def\UMB{Ultrasound in Medecine and Biology}				% 1.252
\def\US{Ultrasonics}							% 1.046
\def\USI{Ultrasonic Imaging}						% 1.409

